Hierarchical Motion Planning under Probabilistic Temporal Tasks and Safe-Return Constraints

Safety is crucial for robotic missions within an uncertain environment. Common safety requirements such as collision avoidance are only state-dependent, which can be restrictive for complex missions. In this work, we address a more general formulation as safe-return constraints, which require the existence of a return-policy to drive the system back to a set of safe states with high probability. The robot motion is modeled as a Markov Decision Process (MDP) with probabilistic labels, which can be highly non-ergodic. The robotic task is specified as Linear Temporal Logic (LTL) formulas over these labels, such as surveillance and transportation. We first provide theoretical guarantees on the re-formulation of such safe-return constraints, and a baseline solution based on computing two complete product automata. Furthermore, to tackle the computational complexity, we propose a hierarchical planning algorithm that combines the feature-based symbolic and temporal abstraction with constrained optimization. It synthesizes simultaneously two dependent motion policies: the outbound policy minimizes the overall cost of satisfying the task with a high probability, while the return policy ensures the safe-return constraints. The problem formulation is versatile regarding the robot model, task specifications and safety constraints. The proposed hierarchical algorithm is more efficient and can solve much larger problems than the baseline solution, with only a slight loss of optimality. Numerical validations include simulations and hardware experiments of a search-and-rescue mission and a planetary exploration mission over various system sizes.

==> contents/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/guo.jpeg}}]{Meng Guo}
(M'11) received the M.Sc. degree (2011) in System, Control, and Robotics
and the Ph.D. degree (2016) in Electrical Engineering from KTH Royal Institute of
Technology, Sweden.
He was a postdoctoral associate with the Department of Mechanical Engineering and Materials Science, Duke University, USA.
During 2018-2021, he worked as a senior research scientist on Reinforcement Learning and Planning at the Bosch Center for Artificial Intelligence (BCAI), Germany.
Since 2022, he is an assistant professor at the Department of Mechanics and Engineering Science, College of Engineering, Peking University, China.
His main research interests include task and motion planning for robotic systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/liao.jpeg}}]{Tianjun Liao}
received the bachelor’s degree from the National University of Defense Technology, Changsha, China, in 2007, and Ph.D. degree from the Institute de Recherches Interdisciplinaires et de Developpements en Intelligence Artificielle, Universite Libre de Bruxelles, Brussels, Belgium, in 2013. He is currently with the Academy of Military Sciences, Beijing, China. His research interests include heuristic optimization algorithms, automated algorithm configuration, and swarm intelligence.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/wang.jpeg}}]{Junjie Wang}
received the B.E. degree (2020) in Automation from Beihang University, Beijing, China.
He is currently a PhD candidate at the College of Engineering, Peking University, China.
His research interests include formal control synthesis for multi-agent systems.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/li.jpeg}}]{Zhongkui Li}
  (M’11, SM’21) received the B.S. degree in space engineering from the National University of Defense Technology, China, in 2005, and his Ph.D. degree in dynamics and control from Peking University, China, in 2010.
  Since 2013, Dr. Li has been with the Department of Mechanics and Engineering Science, College of Engineering, Peking University, China, where he is currently a tenured Associate Professor. He has authored the book \emph{Cooperative Control of Multi-Agent Systems: A Consensus Region Approach} (CRC press, 2014) and has published a number of journal papers. His current research interests include multi-agent systems, autonomous unmanned systems, cooperative control, motion and task planning.
  Dr. Li was the recipient of the State Natural Science Award of China (Second Prize) in 2015, the Yang Jiachi Science and Technology Award in 2015, and the National Excellent Doctoral Thesis Award of China in 2012. His coauthored papers received the \emph{IET Control Theory \& Applications} Premium Award in 2013 and the Best Paper Award of \emph{Journal of Systems Science \& Complexity} in 2012. He serves as an Associate Editor of \emph{IEEE Transactions on Automatic Control}, \emph{Nonlinear Analysis: Hybrid Systems}, and the Conference Editorial Board of IEEE Control Systems Society.
\end{IEEEbiography}

